Progressive Prompts: Continual Learning for Language Models

We introduce Progressive Prompts - a simple and efficient approach for continual learning in language models. Our method allows forward transfer and resists catastrophic forgetting, without relying on data replay or a large number of task-specific parameters. Progressive Prompts learns a new soft prompt for each task and sequentially concatenates it with the previously learned prompts, while keeping the base model frozen. Experiments on standard continual learning benchmarks show that our approach outperforms state-of-the-art methods, with an improvement >20% in average test accuracy over the previous best-preforming method on T5 model. We also explore a more challenging continual learning setup with longer sequences of tasks and show that Progressive Prompts significantly outperforms prior methods.

==> 1_intro.tex <==
Learning a long sequence of tasks without forgetting remains a key feature of human-level intelligence. 
%Mention LLM and their successes
While pretrained language models have largely succeeded in finetuning on a single task, their performance degrades in scenarios where multiple tasks are encountered sequentially, also known as \emph{continual learning} (CL) \citep{de2019episodic, huang2021continual}. A major challenge in CL is \textit{catastrophic forgetting}, i.e., losing the knowledge acquired from previous tasks after learning new ones \citep{mccloskey1989catastrophic, ratcliff1990connectionist}. %\mike{The succeeded vs. fail dichotomy seems a bit strong to me - maybe just say that performance is worse in continual learning than single/multi-task learning?}

%Large-scale language models succeed on a single downstream finetuning task, however their performance degrade when training happens over multiple tasks sequentially. ??? Change this!

% However, training a new model from scratch naively for each task does not solve the forgetting problem \citep{lopez2017gradient}.
% \amjad{forgetting happens because of training from scratch!}



Typical CL approaches for language models use data replay or add a regularization constraint that prevents the model from extensively changing on new tasks \citep{huang2021continual, de2019episodic, sun2019lamol}. These methods, however, still suffer from forgetting due to inevitable changes in parameters shared between tasks. Other approaches, such as progressive networks \citep{rusu2016progressive}, can alleviate catastrophic forgetting completely, but are computationally expensive because they add a new copy of the model for each task. This can be especially intractable for large-scale language models with billions of parameters, which have become a standard in the NLP field \citep{raffel2020exploring}. 

% Then -> parameter-efficient has only been applied to some tasks, now we apply it to progressive nets

% A classical approach to CL is Progressive networks \citep{rusu2016progressive}, which add a neural network (named ``a column'') for each new task, and learn lateral connections from previously learned columns while keeping them frozen. While being quite effective at solving both catastrophic forgetting and forward transfer, progressive networks require training a large number of task-specific parameters for each new task. This can be especially prohibitive for large-scale language models, where each introduced network can have billions of parameters \citep{raffel2020exploring}.

% One class of CL approaches, which are especially effective in avoiding catastrophic forgetting, are the \textit{architectural approaches}. These methods accumulate experiences by adding task-specific parameters for each new task, without modifying previously learned modules \citep{li2019learn, rusu2016progressive, rao2019continual, loo2020generalized}. A classical example of architectural approaches are Progressive Networks \citep{rusu2016progressive}, which add a neural network (a column) for each new task, and learn lateral connections from previously learned columns while keeping them frozen. While being quite effective at alleviating catastrophic forgetting , architectural approaches require training a large number of task-specific parameters. This can be especially prohibitive for large-scale language models, where each introduced network can have billions of parameters \citep{raffel2020exploring}. 

%Recent advances in parameter-efficient learning
% In natural language processing, large-scale pre-trained models have shown strong performance in numerous natural language understanding tasks. However, these models are susceptible to catastrophic forgetting, which is commonly observed during pre-training and finetuning setup, and require a lot of training data. 

%Direct transition to PELT methods ..
% TODO fix this paragraph...
% Recently, there has been substantial progress in tuning pretrained language models by training only a small number of parameters, also known as parameter-efficient language model tuning \citep{li2021prefix, houlsby2019parameter, lester2021power, mao2021unipelt}. Notably, \emph{prompt tuning} \citep{lester2021power} learns a fixed number of tokens, or prompt, to adapt language models on a given downstream task, and can match the quality of fully model finetuning while training $<$0.01\% of the total number of parameters. 

% In this paper, we introduce \textbf{Progressive Prompts} -- a novel CL approach for language models that successfully addresses the issue of catastrophic forgetting. Our approach is inspired by progressive networks, but is significantly more memory-efficient since it adopts prompt tuning -- a separate prompt is learned for each new task and sequentially concatenated with previously learned prompts (Figure~\ref{fig:fig1}). In a straightforward implementation of prompt-based progressive networks for transformer models, each task would have a corresponding trainable prompt prepended to the repeated input embeddings, with future tasks attending to the past tasks' representations. While such a setup allows task-specific input representations, repeating the input becomes infeasible for long task sequences. Hence, we implement a simplified version of the approach, where input tokens are shared across all tasks, while new task prompts are progressively prepended. Our setup allows effective knowledge transfer for future tasks, while preserving the information from the past tasks. To further improve the efficiency of Progressive Prompts, we propose a novel embedding reparameterization technique that enhances prompt tuning performance and allows to shorten the prompt length. 

In this paper, we introduce \textbf{Progressive Prompts} -- a novel CL approach for language models. Our method is inspired by progressive networks, but is significantly more memory-efficient because it only learns a fixed number of tokens, or \emph{prompt}, for each new task. Learning a prompt to adapt language models on a single downstream task was introduced in \emph{prompt tuning} \citep{lester2021power}, and was shown to match the performance of full model finetuning while training $<$0.01\% of the parameters. In Progressive Prompts, we learn a separate prompt for each incoming task and sequentially concatenate it with previously learned prompts. Importantly, we share input tokens across all tasks and progressively prepend new prompts while keeping previous prompts frozen (see Figure~\ref{fig:fig1}). Our method can: 1) alleviate catastrophic forgetting by preserving the knowledge acquired in previous prompts, and 2) transfer knowledge to future tasks by sequentially learning new prompts given previous ones.  %Crucially, previous prompts are kept frozen so we don’t lose information about previous task while training on new tasks. 
%This architecture effectively alleviates catastrophic forgetting in CL for language models, while storing only a very small number of additional parameters (Figure~\ref{fig:fig1}). %Additionally, the sequential addition of prompts allows reusing the knowledge acquired from previous tasks in solving new ones, or forward transfer. 
We also introduce a new technique for prompt embedding reparameterization \citep{li2021prefix}. We show that by passing the prompt embeddings through a residual MLP we can stabilize prompt tuning and improve its performance.


% In this paper, we introduce \textbf{Progressive Prompts} -- a novel CL approach for language models, which combines the power of progressive networks with the efficiency of prompt tuning. Our approach is inspired by progressive networks, but is significantly more memory-efficient since it adopts prompt tuning. The main idea is to learn a separate prompt for each incoming task and sequentially concatenate it with previously learned prompts (Figure~\ref{fig:fig1}). In a straightforward implementation of prompt-based progressive networks, each task would have a corresponding prompt prepended to the repeated input tokens, with future tasks attending to the past tasks' representations (Figure~\ref{fig:fig1}). While such a setup allows task-specific input representations, repeating the input becomes infeasible for long task sequences. Hence, for Progressive Prompts we implement a more efficient setup, where input tokens are shared across all tasks, and new task prompts are progressively prepended. Our method allows effective knowledge transfer for future tasks, and successfully eliminates catastrophic forgetting by preserving prompt parameters from the past tasks.
% We also propose a new technique for prompt embedding reparameterization, which improves prompt tuning performance and allows to decrease the prompt length. 

We run extensive experiments on standard  CL benchmarks for text classification, and show that Progressive Prompts outperforms state-of-the-art approaches on both BERT and T5 architectures \citep{devlin2018bert, raffel2020exploring}. We show over 20\% improvement over the current SOTA for T5 model \citep{qin2021lfpt5}.  
% LFPT5 for CL with T5 model .  
Furthermore, we run experiments on a more challenging CL setup with longer task sequences, and show that our method outperforms prior approaches for T5 and BERT architectures. 




%Finally, the proposed approach is model-agnostic and can be applicable to any transformer-based model. To validate this point, we perform experiments on encoder-based BERT model and encoder-decoder model T5.

%Results, realistic lifelong learning setup with much larger number of tasks than previously explored

Our main contributions in this paper are as follows:
\begin{itemize}
\item We propose a novel CL approach, \emph{Progressive Prompts}, that successfully alleviates catastrophic forgetting, while learning $<0.1\%$ of the total parameters. Furthermore, our method allows knowledge transfer to future tasks from previous ones. 
\item Progressive Prompts is suitable for any transformer-based architecture. We show that it significantly outperforms prior SOTA methods on standard CL benchmarks for both BERT and T5 models. %and requires $<0.1\%$ of trainable parameters in total.
\item We propose a more challenging CL setup encompassing 15 text classification tasks and show that our method significantly outperforms prior methods.
% \item We propose a new technique for improving prompt tuning performance using residual embedding reparameterization. %\amjad{do we want to add this here?}
% BERT and T5.  %\amjad{We show it's suitable for long sequence of tasks.}
% \item no catastrophic forgetting, suitable for long task sequences

\end{itemize}


==> table_lifelong.tex <==

\begin{table}[h!]
\fontsize{9.5}{12}\selectfont
  \begin{center}
    \label{tab:table3}
    \begin{tabular}{lccccccccccccc} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
    \hline
       \textbf{Method} & \multicolumn{3}{c|}{\textbf{7}}  & \multicolumn{3}{c|}{\textbf{6}}  & \multicolumn{3}{c|}{\textbf{3}} & \multicolumn{3}{c|}{\textbf{avg}} \\
       & 20 & 200 & 1000  & 20 & 200 & 1000  & 20, 200 & 1000 & 20 & 200 & 1000 \\
      \hline\hline
      \multicolumn{5}{c}{\textbf{T5-Large results}}  \\
      \hline
      Finetune & 9.3, 8.9, 7.4 & 9.5, 8.1, 7.4 & 10.4, 7.9, 7.5 & 9.7, 8.3, 7.4  \\
      Replay   & 46.0, 45.0, 55.2 & 50.3, 43.7, 54.8 & 34.6, 43.8, 53.3 & 43.6, 44.2, 54.4  \\
      %EWC      & x & x & x & x \\
      PromptTuning & 9.7, 8.4, 8.2 & 24.4, 16.8, 8.7 & 12.2, 8.0, 7.9 & 17.4, 13.9, 10.9 \\
      Per-task Prompts & 69.9, 75.2, 77.0 & 69.9, 75.2, 77.0 & 69.9, 75.2, 77.0 & 69.8, 75.2, 77.0 \\
      LFPT5      & x & x & x & x\\
      ProgPrompt & 75.4, 79.1, 79.5 & 76.6, 78.2, 79.1 & 76.7, 78.9, 79.8 & 76.2, 78.7, 79.5 \\
      \hline
      MTL & x & x & x & x \\
      %\hline 
      %\\BERT-base results
      %\hline
      \hline\hline
      \multicolumn{5}{c}{\textbf{BERT-base results}}  \\
      \hline
      Finetune & 29.9, 43.4, 40.9 & 30.5, 42.0, 42.5 & 33.6, 41.9, 41.8 & x \\
      Replay & 34.9, 46.3, 51.0 & 39.3, 48.1, 51.5  & 34.9, 46.5, 46.3 & 36.4, 47.0, 49.6 \\
      %EWC & x & x & x & x \\
      PromptTuning & x & x & x & x \\
      Per-task Prompts & 50.6, 62.4, 67.2 & 50.6, 62.4, 67.2 & 50.6, 62.4, 67.2 & 50.6, 62.4, 67.2 \\
      IDBR       & 39.7, 48.4, 52.3 & 37.9, 46.6, 54.1 & 32.9, 48.8, 50.1 & 36.8, 47.9, 52.2 \\
      ProgPrompt & 55.3, 67.9, 68.9 & 53.3, 65.8, 70.0 & 51.9, 66.9, 69.0 &  53.5, 66.9, 69.3 \\
      \hline
      MTL & 56.9, 67.7, 69.9 & 56.9, 67.7, 69.9 & 56.9, 67.7, 69.9 & 56.9, 67.7, 69.9
    \end{tabular}
    \caption{Results of lifelong learning experiments with 15 tasks.}
  \end{center}
\end{table}


==> table_t5.tex <==


\begin{table}[h!]
\fontsize{9}{11}\selectfont
  \begin{center}
    \begin{tabular}{lcccccc} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
    \toprule
      &   & \multicolumn{3}{c}{\textbf{Order}}  &  \\
      \textbf{Method} & DR & \textbf{1} & \textbf{2}  & \textbf{3}  & \textbf{avg} \\
      \midrule
      Finetune  & & 18.9 & 24.9 & 41.7 & 28.5  \\
      Replay   & \checkmark &  35.4 & 37.1 & 41.5 & 38.0  \\
      EWC   & &  39.0 & 38.0 & 44.8 & 40.6  \\
      %PromptTuning   & x & x & x & x \\
      LFPT5 & \checkmark &  47.6 & 52.6 & 57.9 & 52.7 \\
      ProgPrompt  & &  \textbf{75.2} & \textbf{75.0} & \textbf{75.1}  & \textbf{75.1}  \\
     \bottomrule
    \end{tabular}
    \caption{Performance on few-shot continual learning benchmark with T5-based CL approaches. DR denotes whether the method requires data replay. All results are averaged over 3 runs.}
    \label{tab:table_t5}
  \end{center}
\end{table}
